Using Illustrations to Communicate Differential Privacy Trust Models: An Investigation of Users' Comprehension, Perception, and Data Sharing Decision

Proper communication is key to the adoption and implementation of differential privacy (DP). However, a prior study found that laypeople did not understand the data perturbation processes of DP and how DP noise protects their sensitive personal information. Consequently, they distrusted the techniques and chose to opt out of participating. In this project, we designed explanative illustrations of three DP models (Central DP, Local DP, Shuffler DP) to help laypeople conceptualize how random noise is added to protect individuals' privacy and preserve group utility. Following pilot surveys and interview studies, we conducted two online experiments (N = 595) examining participants' comprehension, privacy and utility perception, and data-sharing decisions across the three DP models. Besides the comparisons across the three models, we varied the noise levels of each model. We found that the illustrations can be effective in communicating DP to the participants. Given an adequate comprehension of DP, participants preferred strong privacy protection for a certain type of data usage scenarios (i.e., commercial interests) at both the model level and the noise level. We also obtained empirical evidence showing participants' acceptance of the Shuffler DP model for data privacy protection. Our findings have implications for multiple stakeholders for user-centered deployments of differential privacy, including app developers, DP model developers, data curators, and online users.

==> primitive_gau.tex <==
\mypara{Gaussian Mechanism}
\label{subsubsec:gauss}
There are several approaches for designing mechanisms that satisfy $(\epsilon, \delta)$-differential privacy.  In this paper we use the Gaussian mechanism.  The approach computes a function $f$ on the dataset $D$ in a differentially privately way, by adding to $f(D)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_2$ sensitivity of $f$.  Such a mechanism $\AA$ is given below:
$$
\begin{array}{crl}
& \AA(D) & =f(D)+\mathcal{N}\left(\frac{\mathsf{GS}_g\cdot \epsilon}{\sqrt{2\ln(1.25/\delta)}} \right)
  \\
\mbox{where} &  \mathsf{GS}_f & = \max\limits_{(D,D') : D \simeq D'} ||f(D) - f(D')||_2,
\\
\mbox{and}& \Pr{\mathcal{N}\left(\sigma \right)=x} & = \frac{1}{\sqrt{2\pi\sigma}} \myexp{-x^2/2\sigma^2}
\end{array}
$$
In the above, $\mathcal{N}(\sigma)$ denotes a random variable sampled from the normal distribution with mean $0$ and standard deviation $\sigma$, and $\sigma=\sqrt{2\ln(1.25/\delta)}/\epsilon$.
As $\mathcal{N}(\sigma)$ is zero-mean, $\AA(D)$ is a natural (unbiased) estimator of $f(D)$.

==> primitive_grr.tex <==

%\mypara{Randomized Response}
%\label{subsubsec:rr}
% The Gaussian Mechanism can also be applied to ensure LDP, by adding noise $\calN (0, \mathsf{GS}_f^2\cdot \sigma^2 )$ to each single result $f(D) = f(\{v\})$ (e.g., as in~\cite{zheng2017collect}). 
% But for the same (or even better, as Gaussian mechanism have $\delta>0$) privacy guarantee, there exist other mechanisms that gives better utility.  
The basic mechanism in LDP is called random response~\cite{Warner65}.  It was introduced for the binary case, but can be easily generalized to the categorical setting.  Here we present the generalized version of random response (\grr), which enables the estimation of the frequency of any given value $v\in \Domain$.

Here each user with private value $v\in \Domain$ sends the true value $v$ with probability $p$, and with probability $1-p$ sends a randomly chosen $v'\in \Domain$ s.t. $v'\ne v$.  More formally, denote $d$ as the size of the domain $\Domain$, the perturbation function is defined as
\begin{align}
\forall_{y \in \Domain}\;\Pr{\grr(v) = y}  = \left\{
\begin{array}{lr}
p=\frac{e^\epsilon}{e^\epsilon + d - 1}, & \mbox{if} \; y = v  \\
q= \frac{1}{e^\epsilon + d - 1}, & \mbox{if} \; y \neq v \\
\end{array}\label{eq:grr}
\right.
\end{align}
This satisfies $\epsilon$-Local DP since $\frac{p}{q}=e^\epsilon$.  
% Unlike Gaussian mechanism, which adds unbiased noise, random response is asymmetric, and to estimate the frequency of $v\in \Domain$ (i.e., the ratio of the users who have $v$ as private value to the total number of users), one needs to count how many times $v$ is reported, denote by $C(v)$, and then computes
To estimate the frequency of $\tilde{f}_v$ for $v\in \Domain$, one counts how many times $v$ is reported, denoted by $\sum_{i\in[n]}\ind{y_i=v}$, and then computes
\begin{align}
\tilde{f}_v =  \frac{1}{n}\sum_{i\in[n]}\frac{\ind{y_i=v}-q}{p-q} \label{eq:grr_aggregate}
\end{align}
where $\ind{y_i=v}$ is the indicator function that the report of the $i$-th user $y_i$ equals $v$, and $n$ is the total number of users.
%\says{tianhao}{1. we did not cover other mechanisms; 2. each user's contribution is not a one and others zero; 3. some negative values can be made 0}

==> primitive_lap.tex <==
\mypara{Laplace Mechanism}
The Laplace mechanism computes a function $f$ on the dataset $D$ in a differentially private manner, by adding to $f(D)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_f$, the \emph{global sensitivity} or the $\ell_1$ sensitivity of $f$.  When $f$ outputs a single element, such a mechanism $\AA$ is given below:
$$
\begin{array}{crl}
& \AA(D) & =f(D) + \Lapp{\frac{\mathsf{GS}_f}{\epsilon}}
  \\
\mbox{where} &  \mathsf{GS}_f & = \max\limits_{(D,D') : D \simeq D'} ||f(D) - f(D')||_1,
\\
\mbox{and}& \Pr{\Lapp{\beta}=x} & = \frac{1}{2\beta} \myexp{-|x|/\beta}
\end{array}
$$
In the above, $\Lapp{\beta}$ denotes a random variable sampled from the Laplace distribution with scale parameter $\beta$.  When $f$ outputs a vector, $\AA$ adds a fresh sample of $\Lapp{\frac{\mathsf{GS}_f}{\epsilon}}$ to each element of the vector.  In the histogram counting queries, $f(D) = \tuple{\frac{1}{n}\sum \ind{v_i=v}}_{v\in\Domain}$, and $\mathsf{GS}_f = 2/n$, where $\ind{v_i=v}$ is the indicator function that the $i$-th user's value $v_i$ equals $v$ (more generally, $\ind{True}=1$, $\ind{False}=0$).  


